Causality in the Semantics of Esterel: Revisited

We re-examine the challenges concerning causality in the semantics of Esterel and show that they pertain to the known issues in the semantics of Structured Operational Semantics with negative premises. We show that the solutions offered for the semantics of SOS also provide answers to the semantic challenges of Esterel and that they satisfy the intuitive requirements set by the language designers.

==> eptcsdata.tex <==
\providecommand{\event}{B. Klin, P. Soboci\'nski (Eds.): \\
6th Workshop on Structural Operational Semantics (SOS'09)}
\providecommand{\volume}{18}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{32}
\providecommand{\eid}{3}
\pdfoutput=1

